InfiFusion: A Unified Framework for Enhanced Cross-Model Reasoning via LLM Fusion

We introduce InfiFusion, an efficient training pipeline designed to integrate multiple domain-specialized Large Language Models (LLMs) into a single pivot model, effectively harnessing the strengths of each source model. Traditional fusion methods either merge model parameters directly or rely on knowledge distillation with rigid assumptions, limiting their flexibility and efficiency. InfiFusion overcomes these limitations by enhancing Universal Logit Distillation (ULD) with Top-K selection and Logits Standardization. We propose two fusion strategies: Pairwise Fusion (InfiFusion$_p$), where each source model knowledge is distilled individually into the pivot model followed by merging and Unified Fusion (InfiFusion$_u$), where knowledge from all source models is distilled simultaneously into the pivot model. InfiFusion outperforms the state-of-the-art models, such as Qwen-2.5-14B-Instruct and Phi-4, across 11 widely applied benchmarks covering reasoning, coding, mathematics, and instruction-following tasks. Notably, InfiFusion achieves this superior performance while significantly reduces computational costs, completing full training with only 160 H800 GPU hours compared to the millions typically required for traditional LLM training.

==> 3_backup.tex <==



\section{Methods}
\subsection{Preliminary}
We consider a pivot language model (LLM) $M_o$ and $K$ source LLMs $\{M_1, \ldots, M_K\}$, each specializing in distinct domains or tasks. Our objective is to distill the combined strengths of these source models into a single, integrated pivot model $M_o$. Given a dataset $\mathcal{D}$ of instruction--response pairs, we apply knowledge distillation to guide $M_o$ in acquiring complementary expertise from the source models. This process involves defining suitable fusion (distillation) objectives and designing fusion pipelines that integrate diverse knowledge without compromising the overall model quality.

\subsection{Supervised Fine-Tuning (SFT)}
Supervised fine-tuning (SFT) aligns the pivot model $M_o$ with instruction--response pairs in the fine-tuning dataset $\mathcal{D}$. For each instruction $x_i$ and its corresponding response $y_i$ of length $T$, the SFT objective is:
\begin{equation}
\label{eq:sft}
\mathcal{L}_{\text{SFT}} 
= 
-\,\mathbb{E}_{(x_i, y_i) \sim \mathcal{D}} \Bigl[ \sum_{t=1}^{T} \log p_{\theta_o}\bigl(y_{i,t} \mid y_{i,<t}, x_i\bigr) \Bigr],
\end{equation}
where $y_{i,<t}$ denotes the tokens preceding $y_{i,t}$ and $p_{\theta_{o}}(\cdot)$ is the model-predicted token probability under $M_o$.

\subsection{Pairwise Fusion Loss}

A simple way to integrate each source model into the pivot model is \emph{pairwise fusion}: we refine $M_o$ by fusing $M_o$'s outputs with those of a single source $M_j$ at a time. Traditionally, KL-divergence or cross-entropy losses are used in such fusion.
%
However, these conventional measures are sensitive to label mismatches and may fail to accurately capture the differences between probability distributions, particularly when the label space is large or when the supports of the distributions differ. Moreover, KL-divergence is ineffective in handling token alignment.
%
To address these challenges, ~\cite{uld24} proposes replacing KL-divergence with \textit{Universal Logit Distillation Loss} (ULD) loss, a method inspired by Optimal Transport (OT), to better align the distributions and handle mismatches effectively.

\subsubsection{Preliminary}
\paragraph{Optimal Transport Loss}
OT provides a powerful way to compare two discrete distributions by solving a “mass transport” problem. Formally, let 
$p$ and $q$ be two discrete distributions over vocabularies of size 
$V_o$ and $ V_k$, respectively.. We define:
\begin{equation}
\mathrm{OT}(p, q)
= 
\min_{\gamma \in \Pi(p,q)}
\sum_{m=1}^{V_o} \sum_{n=1}^{V_k} \gamma_{m,n} \, C_{m,n}.
\label{eq:ot-def}
\end{equation}
Here, $\Pi(p,q)$ is the set of joint distributions with
marginals $p$ and $q$.
%
The cost matrix $C_{m,n}$ encodes the cost of ``transporting'' one unit of mass from token $m$ to $n$.
%
In practice, Sinkhorn-based methods with entropic regularization can be used to approximate~\eqref{eq:ot-def} efficiently.

\paragraph{Discrete 1-Wasserstein}
An important special case of OT is the 1-Wasserstein distance (also called the Earth Mover’s Distance). In discrete settings, $\mathcal{W}_1(p,q)$ is obtained by choosing a particular cost matrix. For instance, if we set $C_{m,n}=1$ (i.e., uniform cost whenever $m\ne n$), the 1-Wasserstein distance has a closed-form solution:
\begin{equation}
    \mathcal{W}_{1}(p,q)=\sum^{V}_{i=1}|sort(p)_i-sort(q)_i|
\end{equation}
Let $V=\max \bigl(V_o, V_k\bigr)$ be the effective vocabulary size, we augment either the student or teacher vocabulary size through distribution padding (with 0 value), ensuring equal support size for both. 
where $sort(p)$ rearranges the probabilities in 
$p$ in descending order. Intuitively, under uniform cost, the optimal transport simply pairs “largest probability mass” with ``largest probability mass,'' the second-largest with the second-largest, and so on. This makes $\mathcal{W}_1$ particularly simple and effective for aligning distributions whose labels (tokens) may not match one-to-one.


\subsubsection{OT-based Pairwise Fusion Loss}
\label{sec:uld}
In this section, we introduce an OT (Optimal Transport)-based Pairwise Fusion loss to align the predicted distributions from two vocabularies for the same input. Let $M_o$ (pivot model) and $M_k$ (source model) use vocabularies $\mathcal{V}_o$ and $\mathcal{V}_k$, respectively. For an input $x$, we denote its tokenized sequences under $\mathcal{V}_o$ and $\mathcal{V}_k$ by $\Tilde{x}$ and $\hat{x}$, and their parameters by $\theta_o$ and $\theta_k$. 
%
At each time step $t$, $M_o$ produces the conditional distribution $P_{\theta_o}(\cdot \mid \Tilde{x}_{<t})$, while $M_k$ produces $P_{\theta_k}(\cdot \mid \hat{x}_{<t})$, where $\Tilde{x}_{<t}$ and $\hat{x}_{<t}$ are the tokens preceding $t$ in their respective vocabularies. Our goal is to measure and reduce the discrepancy between these distributions, ensuring semantic alignment across the two models.


The ULD loss~\cite{uld24} is a 1-Wasserstein term $\mathcal{W}_1$ that aligns the \emph{entire} probability distributions of $M_o$ and $M_k$. Formally, we define:
\begin{align}
\label{eq:uld}
&\mathcal{L}_{\mathrm{ULD}} =
\sum_{t=1}^{T} \Big[
\mathcal{W}_1\big(
    P_{\theta_o}(\cdot \mid \Tilde{x}_{<t}), 
    P_{\theta_k}(\cdot \mid \hat{x}_{<t})
  \big)
\Big]
\end{align}
However, in this work, we further enhance the semantic interpretation of the cost matrix $C_{m,n}$, allowing more sophisticated formulations. Specifically, to update $M_o$, we replace the conventional KL-based penalty with an OT loss:
\begin{equation}
\label{eq:pair_ot}
\mathcal{L}_{\text{fusion-pair}}^{\mathrm{OT}}
=
\mathbb{E}_{(x_i, y_i) \sim \mathcal{D}}\!\Bigl[
\mathrm{OT}\bigl(P_{\theta_o, i}, P_{\theta_k, i}\bigr)
\Bigr],
\end{equation}
where $C_{m,n} = d(\mathbf{e}_m, \mathbf{e}_n)$, where $\mathbf{e}_m$ and $\mathbf{e}_n$ are token embeddings. This choice of the cost matrix allows us to incorporate richer semantic cues when measuring the distance between tokens in the respective vocabularies.


\subsection{Revised Integrated Fusion Loss}

\paragraph{Top-K Selection and Logit Normalization.}
In this work, we introduce a crucial modification to the conventional knowledge distillation framework: instead of using the entire logit distribution, we focus on the top-k logits for both the student and teacher models. This step is motivated by the observation that, for instruction-based models, the majority of the logits correspond to low-probability categories that contribute little to the distillation process. By selecting only the top `K` logits, we significantly reduce the noise from irrelevant categories, which is particularly beneficial when the logits of the teacher model exhibit a large range of values.

Focusing on the top `K` logits ensures that the student model concentrates on the most informative categories where the probability mass is concentrated. This approach outperforms traditional methods that compare the full sorted logits or probabilities because it avoids the noise introduced by low-probability logits. In practice, for typical instruction models, the top `K` logits (e.g., `K=10`) are sufficient to capture nearly all of the probability mass, making the remaining logits negligible. Additionally, this reduction in the number of logits to compare not only enhances the effectiveness of the distillation process but also improves computational efficiency by sorting and normalizing only the top `K` logits, rather than all logits (e.g., 128k classes).

\paragraph{Logits Standardization.}
We also incorporate a logits standardization as a preprocessing step, which addresses the issue of temperature sharing in conventional knowledge distillation methods. Traditionally, knowledge distillation assumes a shared temperature parameter between the teacher and student models, leading to a forced alignment of logits' magnitudes. This assumption, however, lacks strong theoretical justification, and it can lead to poor performance when the range and variance of logits between the models differ significantly.

Our approach modifies this by applying a logits standardization before the distillation step. This normalization ensures that the student model focuses on the intrinsic relations between the logits of the teacher model rather than attempting to match their magnitudes. The logits standardization helps standardize the logits for each time step, which allows for a more flexible and accurate distillation process. By decoupling the temperature and magnitude of the logits, the student can focus on the relative order of logits and the inherent relationships between them, leading to improved generalization and distillation performance.

The logits standardization procedure is formally defined as follows:
\begin{equation}
\hat{l}_{\text{stu}, t} = \frac{l_{\text{stu}, t} - \mu_{\text{stu}}}{\sigma_{\text{stu}}}, \quad \hat{l}_{\text{tea}, t} = \frac{l_{\text{tea}, t} - \mu_{\text{tea}}}{\sigma_{\text{tea}}},
\end{equation}
where $\mu_{\text{stu}}$ and $\sigma_{\text{stu}}$ are the mean and standard deviation of the logits for the student model, and $\mu_{\text{tea}}$ and $\sigma_{\text{tea}}$ are those for the teacher model, computed over the top-k logits.

\paragraph{Pairwise Fusion Loss with Top-K and Logit Normalization.}
The fusion process between the student model $M_o$ and a teacher model $M_k$ is then performed by computing the Universal Logit Distillation (ULD) loss. After applying the top-k selection and logit normalization, we calculate the ULD loss as follows:
\begin{equation}
\mathcal{L}_{\text{fusion-pair}}^{\text{ULD}} = \mathbb{E}_{(x_i, y_i) \sim \mathcal{D}} \Big[ \sum_{t=1}^{T} \Big| \hat{l}_{\text{stu}, t} - \hat{l}_{\text{tea}, t} \Big| \Big],
\end{equation}
where $T$ is the sequence length. This loss measures the absolute difference between the normalized logits of the student and teacher for each token at each time step, after top-k selection. By minimizing this loss, we encourage the student model to align its predictions with the teacher’s, focusing on the most probable tokens and reducing the impact of irrelevant logits.

\paragraph{Aggregated Fusion Loss from All Teachers.}
To aggregate the knowledge from multiple teacher models, we compute the pairwise fusion loss for each teacher and sum them:
\begin{equation}
\mathcal{L}_{\text{fusion}} = \sum_{k=1}^K \mathcal{L}_{\text{fusion-pair}}^{\text{ULD}, k}.
\end{equation}
This aggregated loss ensures that the student model learns from all teachers simultaneously, incorporating their complementary knowledge while focusing on the most relevant logits as determined by the top-k selection.

\paragraph{Combining with Supervised Fine-Tuning.}
Finally, we combine the fusion loss with the supervised fine-tuning (SFT) loss to form the final objective function:
\begin{equation}
\mathcal{L} = (1 - \lambda) \mathcal{L}_{\text{SFT}} + \lambda \mathcal{L}_{\text{fusion}},
\end{equation}
where $\lambda \in [0, 1]$ controls the relative importance of the supervised training and the distillation process. This formulation ensures that the student model benefits from both labeled data and the distilled knowledge from the teacher models.



% \subsection{Integrated Fusion Loss}
% \paragraph{OT-based Fused Distribution.}
% We propose to first solve for a single \emph{barycenter} distribution $P_{\text{fused}}$ that is close (in OT sense) to all teacher distributions $\{P_{\theta_k}\}_{k=1}^K$:
% \begin{equation}
% P_{\text{fused}}
% =
% \arg\min_{p \in \Delta}
% \sum_{k=1}^K \mathrm{OT}\bigl(P_{\theta_o},\; P_{\theta_k}\bigr).
% \end{equation}
% Here, $\Delta$ is the set of all probability distributions, where each entry is a non-negative number, and the total equals 1. This yields a Wasserstein (or OT) barycenter of the source distributions. Since we directly solve a joint objective over all teachers, we mitigate the risk of \emph{error compounding} that arises from incremental fusion steps.

% \paragraph{Integrated Fusion Objective.}
% Once we obtain $P_{\text{fused}}$, we treat it as the target distribution for the pivot model:
% \begin{equation}
% \mathcal{L}_{\text{fusion-intg}}^{\mathrm{OT}}
% =
% \mathbb{E}_{(x_i,y_i)\sim\mathcal{D}}
% \bigl[
% \mathrm{OT}\bigl(P_{\theta_o, i},\; P_{\text{fused}, i}\bigr)
% \bigr].
% \end{equation}
% By taking gradients of this OT distance with respect to $M_o$'s parameters, we guide $M_o$ to match the fused distribution. This approach simultaneously incorporates the knowledge of all teacher models, without requiring repeated pairwise updates.


% \subsection{Combining Supervised and Fusion Losses}
% Finally, we combine the fusion objectives with the SFT objective:
% \begin{equation}
% \mathcal{L}
% =
% (1 - \lambda)\,\mathcal{L}_{\text{SFT}}
% \;+\;
% \lambda\,\mathcal{L}_{\text{fusion}},
% \end{equation}
% where $\mathcal{L}_{\text{fusion}}$ can be either $\mathcal{L}_{\text{fusion-pair}}^{\mathrm{OT}}$ or $\mathcal{L}_{\text{fusion-intg}}^{\mathrm{OT}}$, depending on the fusion pipeline. The coefficient $\lambda \in [0,1]$ balances the supervised and fusion terms. In addition, different designs of the cost matrix $C_{m,n}$ (e.g., syntactic or semantic distances in the token space) may further improve the reasoning and generalization capabilities of $M_o$.



% \yzy{Note: Replacing KL divergence with OT Loss addresses key limitations of KL in handling sparse, high-dimensional logits with mismatched supports. Unlike KL, OT Loss captures the geometric structure of logits through a cost matrix, enabling robust alignment of distributions even with semantic or syntactic mismatches. This flexibility allows OT Loss to encode task-specific relationships, such as token dependencies or reasoning chains, and to align entire distributions rather than overemphasizing single tokens. Consequently, OT Loss facilitates richer knowledge transfer, harmonizes diverse reasoning styles across teacher models, and enhances the pivot model’s reasoning robustness and generalization.}

% \section{Pairwise Fusion is the Upper Bound of All-in-One}
% In this session, we demonstrate that the performance of pairwise fusion in the upper bound of All-in-One. The loss of All-in-One can be defined as:
% \begin{equation}
% \mathcal{L}_{\text{AiO}} 
% = \lambda_0\mathcal{L}_{\text{SFT}} + \sum_{k=1}^{K} \lambda_k\mathcal{L}_{\theta_k}
% \end{equation}
% where $\sum\lambda_k = 1$, $\mathcal{L}_{\text{SFT}}$ and $\mathcal{L}_{\theta_k}$ is defined in equation \ref{eq:sft} and \ref{eq:uld}, respectively. Therefore, to find the optimal $\theta$ for the All-in-One is to solve the optimization problem:
% \begin{align}
% \theta_{\text{AiO}}^{*} & = \arg\min_{\theta_o} \lambda_0\mathcal{L}_{\text{SFT}} + \sum_{k=1}^{K} \lambda_k\mathcal{L}_{\theta_k}\\
% \end{align}
% In the scenario of the pairwise fusion, we can obtain $\{\theta_{k}^{*}\}_{k=1}^{K}$ fused models, where we have
% \begin{equation}
% \theta_k^{*} = \arg\min_{\theta_o} \beta_k\mathcal{L}_{\text{SFT}} + (1-\beta_k)\mathcal{L}_{\theta_k}.
% \end{equation}
% The final fused model $\theta_{\text{PW}}^{*}$ is derived via weight averaging
% \begin{equation}
%     \theta_{\text{PW}}^{*}  = \sum_{k=1}^{K}\alpha_k\theta_{k}^{*}
% \end{equation}
% where $\sum \alpha_k=1$. In the next steps, we intend to prove that we can always find $\alpha_k, \beta_k, \theta_{\text{PW}}^{*}$ such that
% \begin{equation}
% \mathcal{L}_{\text{AiO}}(\theta_{\text{PW}}^{*}) \leq \mathcal{L}_{\text{AiO}}(\theta_{\text{AiO}}^{*})
% \end{equation}
% Let $\beta_k = 1 - \lambda_k$ and $\alpha_k = \lambda_0/(1-\lambda_k)K$, and we have
% $\lambda_0 = \sum_{k=1}^{K}\alpha_k\beta_k$ and $(1-\beta_k) = \lambda_k$.
% \begin{align}
%     \mathcal{L}_{\text{AiO}}(\theta_{\text{PW}}^{*}) = 
% \end{align}



